Weak Lensing Trispectrum and Kurt-Spectra

We introduce two kurt-spectra to probe fourth-order statistics of weak lensing convergence maps. Using state-of-the-art numerical simulations, we study the shapes of these kurt-spectra as a function of source redshifts and smoothing angular scales. We employ a pseudo-$C_{\ell}$ approach to estimate the spectra from realistic convergence maps in the presence of an observational mask and noise for stage-IV large-scale structure surveys. We compare these results against theoretical predictions calculated using the FFTLog formalism, and find that a simple nonlinear clustering model-the hierarchical ansatz-can reproduce the numerical trends for the kurt-spectra in the nonlinear regime. In addition, we provide estimators for beyond fourth-order spectra where no definitive analytical results are available, and present corresponding results from numerical simulations.

==> local-macro.tex <==
%\oddsidemargin 0in
%\evensidemargin 0in
%\textwidth 7.05in
%\textheight 8.75in
%\hoffset -.15in
%\voffset .4in
%
\def\la{\langle}
\def\ra{\rangle}
\def\n{\noindent}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\ben{\begin{eqnarray}}
\def\een{\end{eqnarray}}
\def\nn{\nonumber}
\def\oh{\bf \hat\Omega}
\def\myC{{\cal C}}
\def\myB{{\cal B}}
\def\myf{\Theta}
\def\bk{{\bf k}}
\def\rtf{r,\theta,\varphi}
\def\br{{\bf r}}
\def\inc{{\int_0^{r_s}}}
\def\rH{\rm H}
\def\myc{{\cal C}}
\def\myC{{\cal C}}
\def\myB{{\cal B}}
\def\myT{{\cal T}}
\def\rD{{\rm D}}
\def\rW{{\rm W}}
\def\add{{_\delta}}
\def\ho{{\hat \Omega}}
\def\ad{{_{\rm{lin}}}}
\def\bk{{\bf k}}
\def\bK{{\bf K}}
\def\bl{{\bf l}}
\def\bx{{\bf x}}
\def\2p{{(2\pi)^2}}
\def\dl{d^2l}
\def\bl{{\bf l}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\ben{\begin{eqnarray}}
\def\een{\end{eqnarray}}
\def\bes{\begin{subequations}}
\def\ees{\end{subequations}}
\def\rpa{{r_{\parallel}}}
\def\rpe{{{\bf r}_{\perp}}}
\def\oh{{\hat\Omega}}
\def\nn{{\nonumber}}
\def\inte{\int_0^{\infty}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
%\newcommand{\edth}{\,\eth\,}
\newcommand{\edthbar}{\,\overline{\eth}\,}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\rA}{{\rm A}}
\def\qtwo{\quad\quad}
\newcommand{\myL}{{\cal L}}
%\newcommand{\calY}{{\cal Y}}
%\newcommand{\calZ}{{\cal Z}}
%\newcommand{\calU}{{\cal U}}
%\newcommand{\calV}{{\cal V}}
%\newcommand{\calW}{{\cal W}}
\newcommand{\rP}{{P}}
\newcommand{\rSZ}{{\rm SZ}}
%\newcommand{\myf}{{\Theta}}
\def\ex{{\int {d^2 {\bf l} \over (2
\pi)^2}~ {\rm P}_{\delta} { \big ( {l\over d_A(r)} \big )} {\rm W}_{\rm TH}^2(l\theta_0)}}
\def\exnew{{\cal J}_{\theta_0}(r)}
\def\ikap0{{\cal J}_{\theta_0}(r)}
\def\ikapp{{\cal J}_{\theta_{12}}(r)}
\def\av{\langle \kappa_{(i)}^2(\theta_0) \rangle}
\def\aviold{\langle \kappa_{(i)}^2(\theta_0) \rangle}
\def\avi{\bar\xi_2^{(i)\kappa}(\theta_0)}
\def\kmin{{\int_0^{r_s}\; \omega_{(i)}(r)\; dr }}
\def\kminnew{{\kappa^{\rm min}_{(i)}}}
\def\one1{\langle \kappa_{(i)}\kappa_{(j)} \rangle}
\def\one{{[\bar \xi^{(ij)}]}}
\def\onei{{[\bar \xi_2^{(i)\kappa}]}}
\def\onej{{[\bar \xi_2^{(j)\kappa}]}}
%
\def\two{\langle \kappa_{\rm }(\oh_1) \kappa_{\rm }(\oh_2) \rangle_c}
\def\two{{[\xi^{(ij)\kappa}_{12}]}}
\def\corr{{{\cal J}_{\theta_{12}}(r)}}
\def\var{{{\cal J}_{\theta_0}(r)}}
\def\oldcorr{\Big [ \int  {d^2 {\bf l} \over (2
\pi)^2 )} {\rm  P}_{\delta}( { {\bf l} \over d_A(r) })  W_{\rm}^2(l\theta_0) \exp [ i l\cdot
\theta_{12}] \Big ]}
\def\oldvar{ \Big [  \int  {d^2 {\bf l} \over (2
\pi)^2 )} {\rm P}_{\delta} ( { {\bf l} \over d_A(r) })  W_{\rm TH}^2(l\theta_0) \Big ] } 
\def\qtwo{\quad\quad}
\def\rsz{{^{\rm SZ}}}
\def\fsky{{f^{-1}_{\rm sky}}}

\def\nfw{(\theta_b)}
\def\fw{\theta_b}
\def\ba{\begin{eqnarray}}
\def\ea{\end{eqnarray}}
\def\f{\frac}
\def\l{\left}
\def\r{\right}
\def\hub{{\cal H}}
\def\nmu{\nabla_{\mu}}
\def\nnu{\nabla_{\nu}}
\def\vp{\varphi}
\def\vt{\vartheta}
%
\def\bk{{\bf k}}
\def\bq{{\bf q}}
\def\rL{{\rm L}}
\def\rD{{\rm D}}
\def\rF{{\rm F}}
%
\def\bell{{\bm\ell}}

\def\pfact{{P_{\delta}(k)P_{\delta}(q_b)}}
\def\tz{\tilde z}



\def\rtf{r,\theta,\phi}
\def\br{{\bf r}}

\def\n{\noindent}
\def\qtwo{\qquad\qquad}
\def\qthree{\qquad\qquad\qquad}



\def\myc{{\cal C}}
\def\myC{{\cal C}}

\def\ad{{_\delta}}
\def\ho{{\hat \Omega}}

\def\bk{{\bf k}}
\def\bK{{\bf K}}

\def\bl{{\bf l}}

\def\bx{{\bf x}}

\def\2p{{(2\pi)^2}}
\def\dl{d^2l}

\def\bl{{\bf l}}

\def\be{\begin{equation}}
\def\ee{\end{equation}}

%ddf

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}

\def\ben{\begin{eqnarray}}
\def\een{\end{eqnarray}}

\def\rpa{{r_{\parallel}}}
\def\rpe{{{\bf r}_{\perp}}}

\def\oh{{\hat\Omega}}
\def\nn{{\nonumber}}

\def\inte{\int_0^{\infty}}

%\def\beqa{\begin{eqnarray}}
%\def\eeqa{\end{eqnarray}}


\def\edth{{\,\eth\,}}
%\newcommand{\edthbar}{\,\overline{\eth}\,}

\def\calX{{\cal X}}
\def\calY{{\cal Y}}
\def\calZ{{\cal Z}}
\def\calU{{\cal U}}
\def\calV{{\cal V}}
\def\calW{{\cal W}}

\def\n{\noindent}
\def\qtwo{\qquad\qquad}
\def\qthree{\qquad\qquad\qquad}

\def\myc{{\cal C}}
\def\myC{{{\cal C}}}
\def\myD{{{\cal D}}}

\def\myB{{\cal B}}

\def\ad{{_\delta}}
\def\ho{{\hat \Omega}}

\def\bk{{\bf k}}
\def\bK{{\bf K}}

\def\bbK{{\rm K}}

\def\bl{{\bf l}}

\def\bx{{\bf x}}

\def\2p{{(2\pi)^2}}
\def\dl{d^2l}
\def\bl{{\bf l}}
\def\neweq{\stackrel{\text{sq}}{\approx}}


\def\kp{{k_{\perp}}}
\def\qp{{q_{3\perp}}}


\def\boh{{\bf{\hat\Omega}}}
\def\bl{{\bf{l}}}


\def\btheta{{\boldsymbol\theta}}

\def\ep{{\boldsymbol\epsilon}}
\def\th{{\boldsymbol\theta}}
\def\ph{{\boldsymbol\phi}}


\def\kp{{\kappa}}
\def\myK{{\cal K}}

